A Journey Among Java Neutral Program Variants

Neutral program variants are functionally similar to an original program, yet implement slightly different behaviors. Techniques such as approximate computing or genetic improvement share the intuition that potential for enhancements lies in these acceptable behavioral differences (e.g., enhanced performance or reliability). Yet, the automatic synthesis of neutral program variants, through speculative transformations remains a key challenge. This work aims at characterizing plastic code regions in Java programs, i.e., the areas that are prone to the synthesis of neutral program variants. Our empirical study relies on automatic variations of 6 real-world Java programs. First, we transform these programs with three state-of-the-art speculative transformations: add, replace and delete statements. We get a pool of 23445 neutral variants, from which we gather the following novel insights: developers naturally write code that supports fine-grain behavioral changes; statement deletion is a surprisingly effective speculative transformation; high-level design decisions, such as the choice of a data structure, are natural points that can evolve while keeping functionality. Second, we design 3 novel speculative transformations, targeted at specific plastic regions. New experiments reveal that respectively 60\%, 58\% and 73\% of the synthesized variants (175688 in total) are neutral and exhibit execution traces that are different from the original.

==> annex.tex <==
\appendix
\section{Appendix}
\label{sec:appendix}

\subsection{Add method invocation}

The following section details the transformation Add method invocation. Listing \ref{lst:addmi-target} describes the subset of the java language targeted, and what follows describes the transformation's behavior.

\lstset{language=Perl,escapeinside={(*@}{@*)},label={lst:addmi-target}}
\begin{lstlisting}
<class> ::= (<modifier>)*
'class' <identifier> (ref)* 
'{' (<class_member>)* '}'

<class_member> ::= <attribute> | 
<other> | <method>

<method> ::= (<modifier>)* (return_type) 
<identifier> '(' 
(<type> <identifier>)* ')' '{' 
(<statement>)* '}'

<statement> ::= <variable_declaration> |
<block> | <other>

<block> ::= (<block_header>) '{' 
(<statement>)* '}'
\end{lstlisting}

$P = \{\text{Packages}\},$

$C(p) = \{\text{Classes of } p \| p \in P\},$

$M(c) = \{\text{methods in class } c\},$ 

$S(m) = \{\text{statements in method } m \text{'s body}\},$ 


$LV(s) = \{\text{Local variables up to } s\},$ 

$Pa(m) = \{\text{Parameter of method } m\},$ 

$A(c) = \{\text{Attributes of class } c\},$ 

$As(c) = \{a \in A(c) \| static(a)\},$ 

Let $p \in P, c \in C(p), m \in M(c), s \in S(m)$

$V(c,m,s) = LV(s) \cup Pa(m) \cup A(c) \cup \{ this \},$
a set of accessible variable from $s$


$Vs(c,m,s) = LV(s) \cup Pa(m) \cup As(c),$
a set of accessible variable from $s$

$\mathcal{M}(p,c,m,s) = \{ m' \in c\} \cup \{ m' \in c' \| \forall c' \in p \land \lnot private(m')\} \cup \{m' \in c' \| \forall p' \in P, \forall c' \in p' \land public(m')\}$

$\mathcal{M}_{a}(p,c,m,s) = \{ m' \| static(m') \lor ClassOf(m') \in TypeOf(LV(c,m,s))\}$

Let $m' \in \mathcal{M}_{a}$

\inference[$\text{Class}$]{
	c\text{ follows } ... m ...
}{
	c -> ... Well;m ...
}

\vspace{1em}

\inference[$\text{Well}_{static \land \lnot void}$]{
	\text{static}(m) \; \; \land \; \; \text{TypeOf}(m') \neq void
}{
	Well -> \text{'public static'} \; \text{TypeOf}(m') \; \text{wellID} 
}

\vspace{1em}

\inference[$\text{Well}_{\lnot static \land \lnot void}$]{
	\lnot \;\text{static}(m) \; \land \; \text{TypeOf}(m') \neq void
}{
	Well -> \text{'public'} \;  \text{TypeOf}(m') \; \text{wellID} 
}

\vspace{1em}

\inference[$\text{Well}_{void}$]{
	\text{TypeOf}(m') = void
}{
	Well -> SKIP
}

\vspace{1em}

\inference[$\text{Method}$]{
	m\text{ follows } ... s ...
}{
	m -> ...  \text{'try \{'} Well \; Ta \; Call; \text{'\} catch (Exception ' eId ') \{\}'} s ...
}
										
\inference[$\text{We}$]{
	\text{TypeOf}(m') \neq void
}
{
	We -> wellID = 
}

\vspace{1em}

\inference[$\text{We}_{void}$]{
	\text{TypeOf}(m') = void
}{
	We -> SKIP
}
%\inference[$\text{We}_{void}$]{
%	\text{TypeOf}(m') \eq void
%}
%{
%	We -> SKIP
%}

\vspace{1em}

\inference[$\text{Target}_{static}$]{
	\text{static}(m')
}{
	Ta -> SKIP
}

\vspace{1em}

\inference[$\text{Target}$]{
	\lnot \; \text{static}(m')
}{
	Ta -> targetID.
}

\vspace{1em}

\inference[$\text{Call}$]{
}{
	Call -> QN(m')(params)
}
																				


\subsection{SwapSubtype}
\label{sec:swap-appendix}
The following section details the behavior of the SwapSubtype transformation, the subset of java targeted \ref{lst:swap-target}, and how it modified it.

\lstset{language=Perl,escapeinside={(*@}{@*)},label={lst:swap-target}}
\begin{lstlisting}
<affectation> ::= <ls> '=' <rs>
<ls> ::=  (<interface> ('<' <type> '>')?)? <identifier>
<rs> ::= 'new' <concrete_class_constructor> ('<' <type> '>')? '(' <param_list> ')'
<param_list> ::= <> | <param> | <param> ',' <param_list>
\label{lst:col-assign}
\end{lstlisting}

$ I = \{\text{Interfaces}\}$

$ T = \{\text{Types}\}$

$ C(t) = \{\text{Constructor of }t\}$

$ T(i) = \{t \in T \| t \text{ implements } i\}$

Let $i \in I, t_{1},t_{2} \in T(i)^2$ such as $t_{1} \neq t_{2}$

\inference[$\text{Affectation}$]{
	\text{Aff}(I,id,t_{1},params) \land \exists c \in C(t_{2}) 
}
{
	\text{Aff}(I,id,t_{1},params) -> I id = 'new' t_{2} '(' params ')'
}

The following sections list the different interfaces targeted by our implementation of the transformation, and for each interface the different classes implementing these interfaces used interchangeably.

\subsubsection{java.util.SortedSet}
\label{sec:col-list}
\begin{itemize}
\item java.util.concurrent.ConcurrentSkipListSet
\item java.util.TreeSet
\end{itemize}
\subsubsection{java.util.concurrent.BlockingDeque}
\begin{itemize}
\item java.util.concurrent.LinkedBlockingDeque
\end{itemize}
\subsubsection{java.util.Collection}
\begin{itemize}
\item java.util.concurrent.LinkedTransferQueue
\item java.util.concurrent.SynchronousQueue
\item java.util.PriorityQueue
\item java.util.concurrent.CopyOnWriteArraySet
\item java.util.concurrent.LinkedBlockingQueue
\item java.util.TreeSet
\item java.util.concurrent.ConcurrentLinkedDeque
\item java.util.Stack
\item java.util.concurrent.PriorityBlockingQueue
\item java.util.ArrayList
\item java.util.HashSet
\item java.util.concurrent.ArrayBlockingQueue
\item java.util.Vector
\item java.util.concurrent.ConcurrentSkipListSet
\item java.util.concurrent.LinkedBlockingDeque
\item java.util.concurrent.DelayQueue
\item java.util.ArrayDeque
\item java.util.LinkedList
\item java.util.LinkedHashSet
\item java.util.concurrent.ConcurrentLinkedQueue
\item java.util.concurrent.CopyOnWriteArrayList
\end{itemize}
\subsubsection{java.util.concurrent.ConcurrentNavigableMap}
\begin{itemize}
\item java.util.concurrent.ConcurrentSkipListMap
\end{itemize}
\subsubsection{java.util.Set}
\begin{itemize}
\item java.util.HashSet
\item gnu.trove.set.hash.THashSet
\item java.util.concurrent.ConcurrentSkipListSet
\item org.apache.commons.collections4.set.ListOrderedSet
\item java.util.concurrent.CopyOnWriteArraySet
\item java.util.TreeSet
\item java.util.LinkedHashSet
\item gnu.trove.set.hash.TCustomHashSet
\end{itemize}
\subsubsection{java.util.concurrent.BlockingQueue}
\begin{itemize}
\item java.util.concurrent.ArrayBlockingQueue
\item java.util.concurrent.LinkedTransferQueue
\item java.util.concurrent.SynchronousQueue
\item java.util.concurrent.LinkedBlockingDeque
\item java.util.concurrent.DelayQueue
\item java.util.concurrent.LinkedBlockingQueue
\item java.util.concurrent.PriorityBlockingQueue
\end{itemize}
\subsubsection{java.util.NavigableSet}
\begin{itemize}
\item java.util.concurrent.ConcurrentSkipListSet
\item java.util.TreeSet
\end{itemize}
\subsubsection{java.util.Deque}
\begin{itemize}
\item java.util.concurrent.LinkedBlockingDeque
\item java.util.ArrayDeque
\item java.util.LinkedList
\item java.util.concurrent.ConcurrentLinkedDeque
\end{itemize}
\subsubsection{java.util.concurrent.TransferQueue}
\begin{itemize}
\item java.util.concurrent.LinkedTransferQueue
\end{itemize}
\subsubsection{java.util.NavigableMap}
\begin{itemize}
\item java.util.concurrent.ConcurrentSkipListMap
\item java.util.TreeMap
\end{itemize}
\subsubsection{java.util.concurrent.ConcurrentMap}
\begin{itemize}
\item java.util.concurrent.ConcurrentSkipListMap
\item java.util.concurrent.ConcurrentHashMap
\end{itemize}
\subsubsection{java.util.List}
\begin{itemize}
\item org.apache.commons.collections4.list.TreeList
\item java.util.Vector
\item org.apache.commons.collections4.list.NodeCachingLinkedList
\item org.apache.commons.collections4.list.CursorableLinkedList
\item java.util.LinkedList
\item org.apache.commons.collections4.list.GrowthList
\item java.util.Stack
\item java.util.ArrayList
\item java.util.concurrent.CopyOnWriteArrayList
\item org.apache.commons.collections4.ArrayStack
\end{itemize}
\subsubsection{java.util.Map}
\begin{itemize}
\item org.apache.commons.collections4.map.SingletonMap
\item org.apache.commons.collections4.map.Flat3Map
\item org.apache.commons.collections4.map.LinkedMap
\item java.util.concurrent.ConcurrentHashMap
\item org.apache.commons.collections4.map.LRUMap
\item org.apache.commons.collections4.map.ListOrderedMap
\item java.util.HashMap
\item org.apache.commons.collections4.map.HashedMap
\item org.apache.commons.collections4.map.ReferenceMap
\item org.apache.commons.collections4.map.CaseInsensitiveMap
\item gnu.trove.map.hash.TCustomHashMap
\item java.util.LinkedHashMap
\item org.apache.commons.collections4.map.PassiveExpiringMap
\item java.util.concurrent.ConcurrentSkipListMap
\item org.apache.commons.collections4.map.StaticBucketMap
\item java.util.TreeMap
\item gnu.trove.map.hash.THashMap
\item java.util.Hashtable
\item java.util.WeakHashMap
\item org.apache.commons.collections4.map.ReferenceIdentityMap
\end{itemize}
\subsubsection{java.util.Iterable}
\begin{itemize}
\item java.util.concurrent.LinkedTransferQueue
\item java.util.concurrent.SynchronousQueue
\item java.util.PriorityQueue
\item java.util.concurrent.CopyOnWriteArraySet
\item java.util.concurrent.LinkedBlockingQueue
\item java.util.TreeSet
\item java.util.concurrent.ConcurrentLinkedDeque
\item java.util.Stack
\item java.util.concurrent.PriorityBlockingQueue
\item java.util.ArrayList
\item java.util.HashSet
\item java.util.concurrent.ArrayBlockingQueue
\item java.util.Vector
\item java.util.concurrent.ConcurrentSkipListSet
\item java.util.concurrent.LinkedBlockingDeque
\item java.util.concurrent.DelayQueue
\item java.util.ArrayDeque
\item java.util.LinkedList
\item java.util.LinkedHashSet
\item java.util.concurrent.ConcurrentLinkedQueue
\item java.util.concurrent.CopyOnWriteArrayList
\end{itemize}
\subsubsection{java.util.Queue}
\begin{itemize}
\item java.util.concurrent.LinkedTransferQueue
\item java.util.concurrent.SynchronousQueue
\item java.util.PriorityQueue
\item java.util.concurrent.LinkedBlockingQueue
\item java.util.concurrent.ConcurrentLinkedDeque
\item java.util.concurrent.PriorityBlockingQueue
\item java.util.concurrent.ArrayBlockingQueue
\item org.apache.commons.collections4.queue.CircularFifoQueue
\item java.util.concurrent.LinkedBlockingDeque
\item java.util.concurrent.DelayQueue
\item java.util.ArrayDeque
\item java.util.LinkedList
\item java.util.concurrent.ConcurrentLinkedQueue
\end{itemize}
\subsubsection{java.util.SortedMap}
\begin{itemize}
\item java.util.concurrent.ConcurrentSkipListMap
\item java.util.TreeMap
\end{itemize}


\subsection{Loopflip}
\label{apx:loopflip}


\lstset{escapeinside={(*@}{@*)},label={lst:loopflip-target}}
\begin{lstlisting}
<loop> ::= 'for(' <initialization> ';'
<condition> ';' <update> ')' '{' 
(<statement>)* '}'

<initialization> ::= <identifier> 
'=' <expression>

<condition> ::= <identifier> 
<binary_operator> <expression>

<binary_operator> ::= '<' |
'<=' | '>' | '>='

<update> ::= <identifier> '=' 
<identifier> <operator> <expression>

<operator> ::= '+' | '(*@-@*)'
\end{lstlisting}
% * | / , == | !=
We extends update statements such as \texttt{i++} into \texttt{i = i + 1} and \texttt{i -= 2} into \texttt{i = i - 2}

$\text{comp} \in \{<,>,\geq,\leq\},\text{op} \in \{+,-\}$

$\overline{a}, \forall a \in  \{<,>,\geq,\leq\} \cup \{+,-\}
\left \{
%\begin{array}{r c l}
\begin{array}{rcl}
>,\geq  & \mapsto & \leq \\
<,\leq   & \mapsto & \geq \\
+ & \mapsto & - \\
- & \mapsto & +
\end{array}
\right .
$


\inference[$\text{For}_{L}$]{
	\text{comp} \in \{\geq,\leq\} \; \land \; |i_{end} - i_{0}| \equiv 0 \pmod p
	}
	{
		(\text{For}_{L}(i=i_{0} i \text{ comp } i_{end} i = i \text{ op } p)-> (\text{For}_{L}(i=i_{end} i \text{ }\overline{\text{comp}}\text{ } i_{0} i = i \text{ }\overline{\text{op}}\text{ } p)
		}
		
		\inference[$\text{For}_{L}$]{
			\text{comp} \not\in \{\geq,\leq\} \; \lor \; \lnot(|i_{end} - i_{0}| \equiv 0 \pmod p)
			}
			{
				(\text{For}_{L}(i=i_{0} i \text{ comp } i_{end} i = i \text{ op } p) -> (\text{For}_{L}(i=i_{end} \; \overline{\text{op}} \;(|i_{end} - i_{0}| \pmod p)  i \text{ }\overline{\text{comp}}\text{ } i_{0} i = i \text{ }\overline{\text{op}}\text{ } p)
				}


==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

The existence of neutral program variants and the ability to generate large quantities of such variants are essential foundations for automatic software improvement. Our work contributes to these foundations with novel empirical facts about neutral variants and with actionable transformations to synthesize such variants. Our empirical analysis explores the space of neutral variants of Java programs, focusing on 6 large open source projects, from different domains. We generated 98225 variants that compile for these projects, through speculative transformations, and 23445 were neutral variants, i.e., more than 20\% of the variants run correctly and pass the same test suite as the original. A detailed analysis of these neutral variants revealed that some language constructs are more prone plastic than others to the synthesis of neutral variants (for example method invocations) and also that some code regions have specific roles that make them plastic (for example optimization code).

The actionable contribution of our work comes in the form of three novel speculative transformations for Java programs. We have designed these transformations to target specific code regions that appear more prone to neutral variant synthesis. Our experiments show that these transformations perform significantly better than generic ones: 60\% (\addmi), 58\% (\swap), 73\% (\loopflip) instead of 23,9\%.

One key insight from the series of experiments reported in this work is that some code regions are \emph{inherently} plastic. These code regions are naturally prone to behavioral variations that preserve the global functionality. These regions include code that has a plastic specification (e.g., hash function); optional functionality (e.g., optimization code) or regions that can be naturally reordered (e.g., loops with no loop-carried dependence). In our future work, we wish to leverage this insight about the deep nature of large programs to develop techniques that can generate vast amounts of software diversity for obfuscation \cite{harrandsoftware} and moving target defenses \cite{Okhravi14moving}.


%Plasticity
% * Language
% * Test
% * Transformations
% 	* ADR random
%    * targeted
% * Traces

==> related.tex <==
\section{Related works}
\label{sec:related}

Our work is related to the seminal work, which analyze the capacity of software at yielding useful variants under speculative transformations. It is also related the works that exploit speculative (either random or targeted) to improve software. 
Here, we discuss the key works in these areas, as well as the novelty of our work.


\subsection{Plasticity of software}

The work on \emph{mutational robustness} by Schulte and colleagues \cite{Schulte13} is a key inspiration for our own work. 
These authors explore the ability of software to be transformed under speculative, random copy, deletion and swap of AST nodes. Their experiments on 22 small to medium C programs (30 to 60 K lines of code) show that 30 \% of the transformations yield variants that are equivalent to the original, modulo the test suite. They call this property of software \emph{mutational robustness}. More recently, this research group demonstrate that the interaction of several neutral mutations can lead a program to exhibit new positive behavior such as passing an additional test. They call this phenomenon \emph{positive epistasis}  \cite{Renzullo2018}.


Our RQ1 can be considered as a conceptual replication \cite{shull_role_2008} of the work by Schulte and colleague. 
Our results mitigate two threats to the validity of Schulte's results: our methodology mitigates internal threats, by using another tool to perform speculative transformations, and our experiment mitigates external threats by transforming Java programs (instead of C). Similarly to Schulte, we conclude ``that mutational robustness is an inherent property of software''. 
Yet, our study also provides completely novel insights about the language constructs and the code areas that support mutational robustness (we call them \emph{plastic code regions}) and about the effectiveness of targeted transformations to maximize the synthesis of neutral variants.

Recently, Danglot and colleagues have also explored the capacity of software and absorbing speculative state transformations \cite{DanglotPBM16}. They explore \emph{correctness attraction}: the extent to which programs can still produce correct results under runtime state perturbations. In that study the authors rely on a perfect oracle to asses the correctness of outputs, and they  observe that many perturbations do not break the correctness in ten subject programs.
Our work also shows that program variants can have different traces and still deliver equivalent results (modulo the test suite). Yet, we rely on different transformations and we analyze in-depth the nature of the code regions that can yield neutral variants.

Our work extends the body of knowledge about forgiving code regions \cite{rinard2012}.
In particular, we find regions characterized by ``plastic specifications'', i.e. regions  which are governed by a very open yet strong contract. For instance, the only correctness contract of a hashing function is to be deterministic. On the one hand this is a strong contract. On the other hand, this is very open: many variants of an hashing function are valid, and consequently, many modifications in the code result in valid hashing functions.

Some recent work investigate a specific form of software plasticity, referred to as \emph{redundancy} \cite{Carzaniga2015,gabel2010study,suzuki2017exploratory}. These works consider that a code fragment is redundant with another fragment, in a specific context, if in that context, both fragments lead a program from a given state to an equivalent one through a different series of intermediate state. 
This is very close to neutral variants, which have diverse visible behavior and yet satisfy the same properties as assessed by the test suite. The key difference between our works is that we investigate speculative transformations to synthesize neutral variants, i.e. increase redundancy, whereas they analyze redundancy that naturally occurs in software systems.


%The entire field of approximate computing propose to trade accuracy for other benefits such as performances. In this case the notion of equivalence is not based on the original test suit anymore but rather on the acceptability of the results\cite{}. But except this difference the field also rely on the detection of region that tolerate to be modified to achieve this trade off. For example, loop perforation\cite{sidiroglou2011} allow to skip the execution of some iteration of some loop in a program. These can be seen as a plastic region.

%In \cite{Hoffmann11}, Hoffmann et al search static configuration parameter in software that they can change the value of in order to obtain a different trade off between accuracy and computational resources used. This parameters that they call Knobs can be seen as plastic regions.

%Approximate computing
%Hoffmann Dynamic Knobs for Responsive Power-Aware Computing
%* transforms static configuration parameters into dynamic knobs
%* Those Knobs are plastic area in a sense
%In \cite{rinard2005}, Rinard defines the notion of \emph{Acceptability Envelope} which is close from \emph{software plasticity} in the context of approximate computing. The main difference is that the notion of equivalence used tolerate that software produce different but still acceptable results. He then propose solution to detect improve and exploit this concept.

%Literature on code clone detection use the concept of Type-4 clone\cite{roy2009comparison,deissenboeck2012challenges,bellon2007comparison}, or semantic clone.  Yet, as noted by Vinayakarao\cite{vinayakarao2018code} semantic clones are different from neutral variants: the latter are expected to exhibit different properties, while the former do not require this aspect. Additionally, this literature on code clones focuses on detecting code snippets that are equivalent, despite eventual syntactic differences. Meanwhile, our work on neutral variants focuses on what factors facilitate the synthesis of an alternative equivalent implementation but that must differ from the original by some properties.


\subsection{Exploiting software plasticity}

Genetic improvement \cite{petke2017genetic} is an area of search-based software engineering \cite{harman2001search}, which consists in automatically and incrementally generating variants of an existing program in order to improve non-functional properties such as resource consumption of execution time. All variants should pass the test suite of the original program.
Existing works in this domain rely on random speculative transformations to search for program variants: Schulte and colleagues \cite{schulte2014} exploit mutational robustness to reduce energy consumption; Langdon et al \cite{langdon2017software} add, delete, replace nodes in C, C++, CUDA ASTs to improve performance;  Cody-Kenny et al. \cite{perfLoc} delete AST nodes, searching for performance improvement; L{\'{o}}pez and colleagues explore program mutations to optimize source code.
All these works leverage the existence of code plasticity, and the performance of the search process can be improved with targeted speculative transformations. In particular, our results with the \swap transformation, show that changing library is very effective to generate neutral variants, and this transformation is a key enabler to improve performance \cite{DBLP:journals/corr/BasiosLWKLB17}.


Software diversification \cite{baudry2015} is the field concerned about the automatic synthesis of program variants for dependability. Existing works in this area also intensively exploit software plasticity and speculative transformations: Feldt \cite{Feldt98} was among the first to  use genetic programming to generate multiple versions of a program to have failure diversity; we relied on random transformations to synthesize diverse implementations of Java programs \cite{Baudry14,allier14}; recent work on composite diversification \cite{wang2017composite}, investigate the opportunity to combine multiple security oriented transformation techniques. These works can benefit from our findings about targeted speculative transformations, which introduce important behavior changes (in particular the \swap transformation), while maximizing the chances of preserving the core functionality.

%Styugin and colleagues\cite{styugin2016new} describe a method transform the application code for both obfuscation purposes and security reasons.

Shacham and colleagues \cite{Shacham} and, more recently, Basios and colleagues \cite{DBLP:journals/corr/BasiosLWKLB17} investigate source code transformations to replace libraries and data structures, in a similar was as the \swap transformation.  This corroborates the idea of a certain plasticity around these data structures, and the notion of interface.



%Approximate computing \cite{mittal2016survey}
%Our work relies on a binary definition of neutral variants (either the variant passes the test suite, or it does not), while Rinard has further explored forgiving code regions to reason about \emph{good enough} software \cite{rinard2005}. In this case, variants under speculative transformation are considered interesting even if the accuracy of the variant is different from the original. This opens the path to approximate computing \cite{sidiroglou2011,Hoffmann11}.





==> results-distance.tex <==



==> results-regions.tex <==
\subsection{RQ1}

bar plot for sosiefication rate on badly tested methods (according to extreme mutation); a couple of bars for each program (one bar for SR on well tested methods and one bar for badly tested methods)

==> results-role.tex <==
\section{RQ2}
